Reference Governor Strategies for Vehicle Rollover Avoidance

The paper addresses the problem of vehicle rollover avoidance using reference governors applied to modify the driver steering input in vehicles with an active steering system. Several reference governor designs are presented and tested with a detailed nonlinear simulation model. The vehicle dynamics are highly nonlinear for large steering angles, including the conditions where the vehicle approaches a rollover onset, which necessitates reference governor design changes. Simulation results show that reference governor designs are effective in avoiding rollover. The results also demonstrate that the controllers are not overly conservative, adjusting the driver steering input only for very high steering angles.

==> Ctrl_SRG.tex <==
%=====================================================================================%
\subsection{\acf{LRG}}
\label{sec:Ctrl_LinearRG}

The \ac{SCG} computes single command value on every update.
As such, the O-infinite set is defined as:
%------- Equation -----------------%
\begin{align}
 \mathcal{O}_{ \infty } &:= \left\{ \left( \mathbf{u}, \mathbf{x} \right) | \mathbf{y}_k = \left( \mathbf{C}  \left( \mathbf{I} - \mathbf{A} \right)^{- 1 } \left( \mathbf{I} - \mathbf{A}^t \right) \mathbf{B} + \mathbf{D} \right) \mathbf{u} +\right.\notag\\
 &\left. \mathbf{C} \mathbf{A}^t \mathbf{x} \in \mathbf{Y}, \forall k \in \mathbb{Z}^{0+} \right\} \subset \mathbb{R}^{4+n}.
 \label{eq:Ctrl_SCG_Oinf}
\end{align}
%------- Equation -----------------%
By applying the O-infinite to the current state, the controller checks if the reference or an alternative command are safe.
If the reference command is dimmed safe, it is passed to the actuator.
If not, the controller selects the alternative safe command that minimizes the difference to the reference one:
%------- Equation -----------------%
\begin{align}
 \mathbf{v} &= \argmax_{ \mathbf{v} } \left\{ k_{CG} | \mathbf{v} = \mathbf{v}_{k - 1} + k_{CG} \left( \mathbf{u}_{k} - \mathbf{v}_{k - 1} \right), \right. \notag\\
  &\left. \left( \mathbf{v}, \mathbf{x} \right) \in \mathcal{O}_{ \infty } \: \mathsf{and} \: k_{CG} \in \left[ 0, 1 \right] \right\},
 \label{eq:Ctrl_SCG_Cmd}
\end{align}
%------- Equation -----------------%
where $ \mathbf{u}_{k} $ is the current reference command and $ \mathbf{v}_{k - 1} $ is the previous command used.

\begin{remark}
 Because the command governor checks at each update if a command is safe for the future steps, $ \mathbf{v}_{k - 1} $ is known to be safe for the current step.
 As such, in the optimization process \eqref{eq:Ctrl_SCG_Cmd} only needs to analyze the interval $ \mathbf{u} \in \left[ \mathbf{u}_{k}, \mathbf{v}_{k - 1} \right] $.
\end{remark}

%\begin{enumerate}
% \item Command Governor activation logic
% 
% \item Command dynamics (when the Command Governor is active)
% 
% \item Constraint admissible sets
% 
% \item Command selection method
%\end{enumerate}




